Joint Energy-based Model Training for Better Calibrated Natural Language Understanding Models

In this work, we explore joint energy-based model (EBM) training during the finetuning of pretrained text encoders (e.g., Roberta) for natural language understanding (NLU) tasks. Our experiments show that EBM training can help the model reach a better calibration that is competitive to strong baselines, with little or no loss in accuracy. We discuss three variants of energy functions (namely scalar, hidden, and sharp-hidden) that can be defined on top of a text encoder, and compare them in experiments. Due to the discreteness of text data, we adopt noise contrastive estimation (NCE) to train the energy-based model. To make NCE training more effective, we train an auto-regressive noise model with the masked language model (MLM) objective.

==> data_implementation.tex <==
\section{Data-sets and Implementation Details}
\label{sec:data_implement}

%In this section we describe data-sets and implementation details.

\subsection{Data-sets}
\label{sec:datasets}

For pre-training, we use the large-scale CCNEWS data \cite{anton19realfake} which is a de-duplicated subset of the English portion of the CommonCrawl news data-set\footnote{
\url{http://commoncrawl.org/2016/10/news-dataset-available}
}.
The dataset contains news articles published worldwide between September 2016 and February 2019. It has in total around 1 billion sentences or 27 billion words. To be able to complete experiments in a reasonable amount of time, we use the first 10 percent of the CCNEWS data for pre-training, which contains 100 million sentences and 2.7 billion words. 
%We refer to it by CCNEWS-100m in the writing of this paper.

For fine-tuning, three open-domain conversational dialogue data-sets are used: Dailydialog (1.3 million words) \cite{dailydialog17yanran}, Switchboard (1.2 million words), and Cornell Movie \cite{cornell11cristian} (4.5 million words). To save space, we defer the details of the data-sets to Appendix \ref{appsec:dataset}.

To construct the vocabulary, we learn codes of Byte Pair Encoding (BPE) \cite{bpe16sennrich} from the CCNEWS-100m data with 50k merges. This results in a vocabulary of size 62k. We then apply the same BPE codes to all target dialogue data-sets.  

\subsection{Implementation}

Our code is based on the Fairseq toolkit \cite{ott2019fairseq}. The Adam optimizer \cite{adam14kingma} is used for all experiments. For pre-training of both MASS and NS, we use a mini-batch size of 2048, with the learning rate (LR) set to 0.0001. Following \cite{tfattention17Vaswani}, the ``inverse square root'' LR scheduler with a warm-up stage is used. Pre-training is conducted on 32 GPUs and half-precision (float16) speed-up is used. For both MASS and NS, we stop the pre-training after the CCNEWS data is swept 20 times.  For all our experiments, a dropout rate of 0.1 is applied to the transformer model. We follow \cite{song2019mass} for the recommended hyper-parameter setting of MASS (e.g. how to select the mask span).
%Although the perplexity is still improving, we stop the pre-training for practical reasons to control the duration of the experiments.
%(with or without mix-review)

Fine-tuning is done on 2 GPUs without float16 speed-up. The learning rate is halved when the PPL on the validation set does not improve. In almost all fine-tuning experiments over-fitting is observed, and we do an early-stop when performance on the validation set starts to deteriorate. We tune the learning rate from \{$10^{-3}$,$10^{-4}$,$10^{-5}$\}, and report the best model based on validation set perplexity.

%Moreover, we believe the additional pre-training data used during mix-review is not going to make a visible difference on PPL, the reason is that the fine-tuning is only run for a few epochs, and only a small mix-ratio is used. Take the Dailydialogue experiment for example, we calculate that  mix-review only uses 2\% of the pre-training data, which is negligible comparing to the computing (swept for 20 times) used in pre-training.


==> eacl2021_rebutall.tex <==
General: 

We sincerely thank all reviewers for their insightful comments! Please refer to our responses to individual reviewers.

#1

Thanks for the review! Here's our response to the concerns or questions:

Re "while improvements in ECE seem significant, the paper does not present which impact this may have in practice.":

A: Calibration has been regarded as an important issue for deep learning models (https://arxiv.org/abs/1706.04599), and we have provided concrete examples (Table 2&5) that the EBM trained model tends to give more conservative predictions for high-energy samples (implicating this sample could be out-of-distribution).

Re "from figure 3, it seems that Roberta is initially well-calibrated, and fine-tuning causes this to deteriorate. ":

A: We explained (line 345) that the calibration for baseline becomes worse as it reaches high-accuracy area (late stage in the training iterations). And in our analysis (Figure 2 or Table 2), we have shown that the baseline model become poorly calibrated because it gives overly confident prediction.

Re "why do you use a GPT-2 model (with MLM) instead of a BERT-like model (like ELECTRA did)":

A: Good question. We explained in Appendix B that, due to the nature of masked language modeling and the bi-directional architecture of BERT /Roberta, the sampled tokens will be independent of each other, which could result in unnatural and easy-to-detect noise samples. That is why we choose to utilize an auto-regressive LM (e.g., GPT-2). We acknowledge this design choice complicates our framework a bit. The setting in ELECTRA (which uses a BERT-like noise model) is different in that it's a token-level discriminator, however in our case NCE is done on sentence-level.

Re "You instead refer to P_N terms "which could be of very small value, this specific issue has been adressed in 'Learning with Noise-Contrastive Estimation: Easing training by learning to scale' (COLING 2018), with a description of why substracting log(P_N) mitigates the problem.":

A: Thanks for referring us to that paper! We suppose you are referring to " initializing output bias with values of log P_N(w) gives even better results" in Sec4.4 of https://www.aclweb.org/anthology/C18-1261.pdf . Note that in our work, NCE is applied on sentence-level, instead of word level. Therefore, unlike their work, our model do not have output bias associated to each token (or each sample). We agree that this is an intriguing and valuable paper on NCE, but whether that technique can benefit our work is unknown. We have added this citation to the manuscript.

Re typos:

Thank you for pointing those out! We have fixed them in the manuscript.

#2

Thanks for the review! Here's our response to the concerns or questions:

Re "Do these results infer that, while for optimizing during train, EBM is superior in terms of calibration, it is somewhat on par to a system that was trained on an additional dev set?":

A: Yes your understanding is correct. 

Re Fig. 2 hard to read:

A: Sorry about that. We will provide an enlarged version of that figure in the updated version of the manuscript.

Re "l 335 mentions significant improvements - on what confidence? ":

A: We simply mean "significant" in its literal meaning (non-statistical) :) More specifically, we mean that the relative improvement for the ECE metric is large.


#3

Thanks for the review! Here's our response to the concerns or questions:

Re "Eq. 4 ... - LogSumExp (f_CLS(enc(x))). That is, drop the "y" subscript on LogSumExp. it is unbound and doesn't make sense. Put another way, LogSumExp is a function of the entire set of logits, and returns a scalar without a need for an argument y.":

A: Thanks for the suggestion, but we were following the notations from https://arxiv.org/pdf/1912.03263.pdf. You can interpret the subscript "y" in the same way as subscripts in the common summation \sum(_y) operations. To make it more clear, we have put bounds to the formulation in the updated version of the manuscript.

Re "Paragraph 2.4 ... Please expand this section in the new version of the paper. There are multiple possible interpretations.":

A: Thanks for the suggestion! We will move the explanations in Appendix B to the main part for better clarification.

==> trash.tex <==
\begin{table}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{tabular}{l|l}
\hline
News & Dialogue \\
\hline
\textbf{Context Input:} the avengers are super hot currently .  & \textbf{Context Input:} what did you do yesterday ?  \\ 
 \texttt{<eou>} the next movie will be on in April . & \texttt{<eou>} i watched the avengers movie . \\
\textbf{Target Output:} fans are talking about what & \textbf{Target Output:} wow ! i am crazy \\
what iron man will do on the internet . &  about iron man ! \\
\hline
\end{tabular}
\end{small}
\caption{Examples our input-output pairs. Left: Next-sentence pre-training with news data. Right: Normal dialogue response model training.}
\label{tab:illustrate-ns}
\end{center}
\vskip -0.1in
\end{table}

